JAX-Fluids 2.0: Towards HPC for Differentiable CFD of Compressible Two-phase Flows

In our effort to facilitate machine learning-assisted computational fluid dynamics (CFD), we introduce the second iteration of JAX-Fluids. JAX-Fluids is a Python-based fully-differentiable CFD solver designed for compressible single- and two-phase flows. In this work, the first version is extended to incorporate high-performance computing (HPC) capabilities. We introduce a parallelization strategy utilizing JAX primitive operations that scales efficiently on GPU (up to 512 NVIDIA A100 graphics cards) and TPU (up to 1024 TPU v3 cores) HPC systems. We further demonstrate the stable parallel computation of automatic differentiation gradients across extended integration trajectories. The new code version offers enhanced two-phase flow modeling capabilities. In particular, a five-equation diffuse-interface model is incorporated which complements the level-set sharp-interface model. Additional algorithmic improvements include positivity-preserving limiters for increased robustness, support for stretched Cartesian meshes, refactored I/O handling, comprehensive post-processing routines, and an updated list of state-of-the-art high-order numerical discretization schemes. We verify newly added numerical models by showcasing simulation results for single- and two-phase flows, including turbulent boundary layer and channel flows, air-helium shock bubble interactions, and air-water shock drop interactions.

==> figures/air_helium_shockbubble/2D/flowfields.tex <==
\begin{tikzpicture}

    \node at (0cm,7cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/levelset_128_2D.png}};
    \node at (8cm,7cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/diffuse_128_2D.png}};
    \node at (0cm,4cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/levelset_256_2D.png}};
    \node at (8cm,4cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/diffuse_256_2D.png}};
    \node at (0cm,1cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/levelset_512_2D.png}};
    \node at (8cm,1cm) {\includegraphics[scale=0.5]{figures/air_helium_shockbubble/2D/flowfields/diffuse_512_2D.png}};
    % \node at (10cm,3.9cm) {(b)};
    % \node at (10cm,3.9cm) {(b)};

\end{tikzpicture}

==> figures/gradients/verification_2D/contour.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cyan}{RGB}{0,255,255}
\definecolor{magenta}{RGB}{255,0,255}
\definecolor{mediumslateblue128127255}{RGB}{128,127,255}

\newcommand{\myLineWidth}{0.75pt}

\begin{axis}[
    tick align=outside,
    tick pos=left,
    xmin=-1, xmax=2,
    ymin=-1, ymax=1,
    axis equal image,
    xlabel={$x / D_0$},
    ylabel={$y / D_0$},
]
\addplot [draw=black, dotted, line width=0.75pt]
table{figures/gradients/verification_2D/contour-000.dat}; \label{pgfplots:eb0}
\addplot [draw=black, line width=0.75pt]
table{figures/gradients/verification_2D/contour-001.dat}; \label{pgfplots:eb1}
\addplot [draw=black, dashed, line width=0.75pt]
table{figures/gradients/verification_2D/contour-002.dat}; \label{pgfplots:eb2}

\addplot [dotted, draw=cyan, line width=0.75pt]
table{figures/gradients/verification_2D/contour-003.dat};
\addplot [draw=cyan, line width=0.75pt]
table{figures/gradients/verification_2D/contour-004.dat}; \label{pgfplots:Ms0}
\addplot [dashed, draw=cyan, line width=0.75pt]
table{figures/gradients/verification_2D/contour-005.dat};

\addplot [dotted, draw=mediumslateblue128127255, line width=0.75pt]
table{figures/gradients/verification_2D/contour-006.dat};
\addplot [draw=mediumslateblue128127255, line width=0.75pt]
table{figures/gradients/verification_2D/contour-007.dat}; \label{pgfplots:Ms1}
\addplot [dashed, draw=mediumslateblue128127255, line width=0.75pt]
table{figures/gradients/verification_2D/contour-008.dat};

\addplot [dotted, draw=magenta, line width=0.75pt]
table{figures/gradients/verification_2D/contour-009.dat};
\addplot [draw=magenta, line width=0.75pt]
table{figures/gradients/verification_2D/contour-010.dat}; \label{pgfplots:Ms2}
\addplot [dashed, draw=magenta, line width=0.75pt]
table{figures/gradients/verification_2D/contour-011.dat};
\end{axis}

\end{tikzpicture}


==> figures/gradients/verification_2D/gradient_.tex <==
% \begin{tikzpicture}
% \begin{axis}[enlargelimits=false]
%     \addplot [
%         matrix plot*,
%         nodes near coords=\coordindex,mark=*,
%         mesh/cols=3,
%         mesh/rows=3,
%         point meta=explicit,
%         mesh/ordering=y varies,
%     % ] table [meta=grad0] {
%     %     Ms eb grad0
%     %     1.1000000000000001 -0.5000000000000000 6.0854177659520783
%     %     1.1000000000000001 0.0000000000000000 6.2699677109651724
%     %     1.1000000000000001 0.5000000000000000 6.4547241326409317
%     %     1.3000000000000000 -0.5000000000000000 4.1783097335171773
%     %     1.3000000000000000 0.0000000000000000 4.1429422904364612
%     %     1.3000000000000000 0.5000000000000000 4.0986917547080743
%     %     1.5000000000000000 -0.5000000000000000 3.4865082554842566
%     %     1.5000000000000000 0.0000000000000000 3.7266785312119888
%     %     1.5000000000000000 0.5000000000000000 4.1351654538673497        
%     % };
%     ] table[meta=grad0] {figures/gradients/verification_2D/plot_data_0.txt};
% \end{axis}
% \end{tikzpicture}

\begin{tikzpicture}
    \begin{groupplot}[
        group style={group size=2 by 2}, 
        width=5.5cm, 
        height=5.5cm
    ]
    \nextgroupplot[enlargelimits=false]
    \addplot [
        matrix plot*,
        mesh/cols=21,
        mesh/rows=21,
        point meta=explicit,
        mesh/ordering=y varies,
    ] table[meta=grad0] {figures/gradients/verification_2D/plot_data_0.txt};

    \nextgroupplot[enlargelimits=false]
    \addplot [
        matrix plot*,
        mesh/cols=21,
        mesh/rows=21,
        point meta=explicit,
        mesh/ordering=y varies,
    ] table[meta=grad0] {figures/gradients/verification_2D/plot_data_1.txt};

    \nextgroupplot[enlargelimits=false]
    \addplot [
        matrix plot*,
        mesh/cols=21,
        mesh/rows=21,
        point meta=explicit,
        mesh/ordering=y varies,
    ] table[meta=grad0] {figures/gradients/verification_2D/plot_data_2.txt};

    \nextgroupplot[enlargelimits=false]
    \addplot [
        matrix plot*,
        mesh/cols=21,
        mesh/rows=21,
        point meta=explicit,
        mesh/ordering=y varies,
    ] table[meta=grad0] {figures/gradients/verification_2D/plot_data_3.txt};
\end{groupplot}
\end{tikzpicture}

==> figures/scaling/mean_std_times.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}

\pgfplotsset{ every non boxed x axis/.append style={x axis line style=-},
     every non boxed y axis/.append style={y axis line style=-}}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=2cm}, width=7cm, height=7cm]
\nextgroupplot[
log basis x={2},
log basis y={2},
title=(a),
tick align=outside,
tick pos=left,
xlabel={nodes},
xmin=0.784584097896751, xmax=163.143760296866,
xmode=log,
xtick={1,2,4,8,16,32,64,128},
xticklabels={1,2,4,8,16,32,64,128},
ytick={32,128,512,2048},
y tick style={color=blue},
y tick label style={color=blue},
ylabel=\textcolor{blue}{mean},
ymin=16, ymax=4096,
ymode=log,
legend style={at={(0.95,0.05)},draw=none,anchor=south east},
ytick style={color=blue}
]

\addplot [semithick, blue, mark=*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/singlephase_tpu.txt};
\addlegendentry{SP};

\addplot [semithick, blue, dashed, mark=x, mark size=2, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/diffuse_tpu.txt};
\addlegendentry{DI};

\addplot [semithick, blue, dash dot, mark=square*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/levelset_tpu.txt};
\addlegendentry{LS};

\nextgroupplot[
log basis x={2},
log basis y={2},
tick align=outside,
tick pos=left,
xlabel={nodes},
xmin=0.784584097896751, xmax=163.143760296866,
xmode=log,
xtick={1,2,4,8,16,32,64,128},
xticklabels={1,2,4,8,16,32,64,128},
ytick={32,128,512},
y tick style={color=blue},
y tick label style={color=blue},
ymin=16, ymax=1024,
ymode=log,
ytick style={color=blue}
]
\addplot [semithick, blue, mark=*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/singlephase_gpu.txt};

\addplot [semithick, blue, dashed, mark=x, mark size=2, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/diffuse_gpu.txt};

\addplot [semithick, blue, dash dot, mark=square*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {1}
] {figures/scaling/levelset_gpu.txt};
\end{groupplot}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=2cm}, width=7cm, height=7cm]
\nextgroupplot[
axis y line=right,
log basis x={2},
log basis y={2},
tick align=outside,
xmin=0.784584097896751, xmax=163.143760296866,
xmode=log,
xtick pos=left,
ymin=0.006, ymax=16,
ymode=log,
ytick pos=right,
ytick style={color=green01270},
xtick={},
xticklabels={},
ytick={0.015625,0.0625,0.25,1,4},
yticklabel style={anchor=west, color=green01270}
]
\addplot [semithick, green01270, mark=*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/singlephase_tpu.txt};

\addplot [semithick, green01270, dashed, mark=x, mark size=2, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/diffuse_tpu.txt};

\addplot [semithick, green01270, dash dot, mark=square*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/levelset_tpu.txt};

\nextgroupplot[
axis y line=right,
log basis x={2},
log basis y={2},
tick align=outside,
xmin=0.784584097896751, xmax=163.143760296866,
xmode=log,
xtick pos=left,
ymin=0.006, ymax=16,
ymode=log,
title=(b),
ytick pos=right,
ytick style={color=green01270},
ylabel=\textcolor{green01270}{std},
xtick={},
xticklabels={},
ytick={0.015625,0.0625,0.25,1,4},
yticklabel style={anchor=west, color=green01270},
]

\addplot [semithick, green01270, mark=*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/singlephase_gpu.txt};

\addplot [semithick, green01270, dashed, mark=x, mark size=2, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/diffuse_gpu.txt};

\addplot [semithick, green01270, dash dot, mark=square*, mark size=1, mark options={solid}] table[
    x index = {0}, y index = {2}
] {figures/scaling/levelset_gpu.txt};


\end{groupplot}

\end{tikzpicture}


==> figures/spatial_reconstruction_schematic.tex <==
\begin{tikzpicture}
    \coordinate (IMM) at (-3,0);
    \coordinate (IM) at (-1.5,0);
    \coordinate (I) at (0,0);
    \coordinate (IP) at (1.5,0);
    \coordinate (IPP) at (3,0);
    \coordinate (IPPP) at (4.5,0);
    
    \draw (IMM) -- (IPPP);
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i-2$] at (IMM) {};
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i-1$] at (IM) {};
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i$] at (I) {};
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i+1$] at (IP) {};
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i+2$] at (IPP) {};
    \node [circle,fill=black,inner sep=1pt,label=below:\strut$i+3$] at (IPPP) {};

    \draw [dashed] ($0.5*(I) + 0.5 *(IP) + (0.0,0.5)$) node [above] {$i + \frac{1}{2}$} -- ($0.5*(I) + 0.5*(IP) + (0.0,-4.25)$);

    \draw ($(IMM) + (0.0,-1.0)$) -- ($(I) + (0.0,-1.0)$);
    \node [circle,fill=black,inner sep=1pt] at ($(IMM) + (0.0,-1.0)$) {};
    \node [circle,fill=black,inner sep=1pt] at ($(IM) + (0.0,-1.0)$) {};
    \node [circle,fill=black,inner sep=1pt,label=below right:$S_0$] at ($(I) + (0.0,-1.0)$) {};

    \draw ($(IM) + (0.0,-2.0)$) -- ($(IP) + (0.0,-2.0)$);
    \node [circle,fill=black,inner sep=1pt] at ($(IM) + (0.0,-2.0)$) {};
    \node [circle,fill=black,inner sep=1pt] at ($(I) + (0.0,-2.0)$) {};
    \node [circle,fill=black,inner sep=1pt,label=below right:$S_1$] at ($(IP) + (0.0,-2.0)$) {};

    \draw ($(I) + (0.0,-3.0)$) -- ($(IPP) + (0.0,-3.0)$);
    \node [circle,fill=black,inner sep=1pt] at ($(I) + (0.0,-3.0)$) {};
    \node [circle,fill=black,inner sep=1pt] at ($(IP) + (0.0,-3.0)$) {};
    \node [circle,fill=black,inner sep=1pt,label=below right:$S_2$] at ($(IPP) + (0.0,-3.0)$) {};

    \draw ($(I) + (0.0,-4.0)$) -- ($(IPPP) + (0.0,-4.0)$);
    \node [circle,fill=black,inner sep=1pt] at ($(I) + (0.0,-4.0)$) {};
    \node [circle,fill=black,inner sep=1pt] at ($(IP) + (0.0,-4.0)$) {};
    \node [circle,fill=black,inner sep=1pt] at ($(IPP) + (0.0,-4.0)$) {};
    \node [circle,fill=black,inner sep=1pt,label=below right:$S_3$] at ($(IPPP) + (0.0,-4.0)$) {};

\end{tikzpicture}
